Statistical multi-metric evaluation and visualization of LLM system predictive performance

The evaluation of generative or discriminative large language model (LLM)-based systems is often a complex multi-dimensional problem. Typically, a set of system configuration alternatives are evaluated on one or more benchmark datasets, each with one or more evaluation metrics, which may differ between datasets. We often want to evaluate -- with a statistical measure of significance -- whether systems perform differently either on a given dataset according to a single metric, on aggregate across metrics on a dataset, or across datasets. Such evaluations can be done to support decision-making, such as deciding whether a particular system component change (e.g., choice of LLM or hyperparameter values) significantly improves performance over the current system configuration, or, more generally, whether a fixed set of system configurations (e.g., a leaderboard list) have significantly different performances according to metrics of interest. We present a framework implementation that automatically performs the correct statistical tests, properly aggregates the statistical results across metrics and datasets (a nontrivial task), and can visualize the results. The framework is demonstrated on the multi-lingual code generation benchmark CrossCodeEval, for several state-of-the-art LLMs.

==> prior.tex <==
\section{Prior work
\label{sec:prior_work}}

\cite{dror2020statistical}[chap. 6] present a framework for statistical system comparison across multiple datasets.  Using adjustment of p-values for multiple hypotheses (see Section~\ref{ssec:order_of_comparisons}), they propose hypothesis tests of whether one system is superior to another in at least $u\geq 1$ (user-specified) out of $N$ datasets considered, and to identify which datasets these are.
